Deep Spectral Improvement for Unsupervised Image Instance Segmentation

Deep spectral methods reframe the image decomposition process as a graph partitioning task by extracting features using self-supervised learning and utilizing the Laplacian of the affinity matrix to obtain eigensegments. However, instance segmentation has received less attention compared to other tasks within the context of deep spectral methods. This paper addresses the fact that not all channels of the feature map extracted from a self-supervised backbone contain sufficient information for instance segmentation purposes. In fact, Some channels are noisy and hinder the accuracy of the task. To overcome this issue, this paper proposes two channel reduction modules: Noise Channel Reduction (NCR) and Deviation-based Channel Reduction (DCR). The NCR retains channels with lower entropy, as they are less likely to be noisy, while DCR prunes channels with low standard deviation, as they lack sufficient information for effective instance segmentation. Furthermore, the paper demonstrates that the dot product, commonly used in deep spectral methods, is not suitable for instance segmentation due to its sensitivity to feature map values, potentially leading to incorrect instance segments. A new similarity metric called Bray-Curtis over Chebyshev (BoC) is proposed to address this issue. It takes into account the distribution of features in addition to their values, providing a more robust similarity measure for instance segmentation. Quantitative and qualitative results on the Youtube-VIS2019 dataset highlight the improvements achieved by the proposed channel reduction methods and the use of BoC instead of the conventional dot product for creating the affinity matrix. These improvements are observed in terms of mean Intersection over Union and extracted instance segments, demonstrating enhanced instance segmentation performance. The code is available on: https://github.com/farnooshar/SpecUnIIS

==> temp/temp_introduction.tex <==
\IEEEPARstart{P}ixel-wise classification problem is referred to as semantic segmentation. This task aims to assign a specified class (or label) to each pixel in an image. It is a fundamental topic in the field of computer vision, and it can be applied to a wide variety of applications in the real world, including virtual reality,  autonomous driving, and video surveillance. Various semantic segmentation approaches have recently emerged based on deep neural networks that have shown superior performance. The succeeding methods, such as DeepLab \cite{chen2017rethinking} and PSPNet \cite{zhao2017pyramid}, have achieved a considerable improvement in the accuracy of segmentation, albeit they frequently include cumbersome models and costly computation.

Some real-time architectures for semantic segmentation have been proposed to tackle this problem, e.g., ENet \cite{paszke2016enet}, ESPNet \cite{mehta2018espnet}, ICNet \cite{zhao2018icnet} and BiSeNet \cite{yu2018bisenet}\cite{yu2021bisenet}.
On the other hand, several strategies have been proposed to reduce the model's size and improve its cost-effectiveness, including model pruning, model quantization, and knowledge distillation. Among these, knowledge distillation is currently being researched in depth. Knowledge distillation refers to the method that helps the training process of a smaller network (student) under the supervision of a more extensive network (teacher) which was first proposed in \cite{hinton2015distilling}. Unlike other compression methods, it can reduce the size of a network without consideration of the structural differences that exist between a teacher network and a student network.

\begin{figure}[t]
\begin{flushright}
{\includegraphics[scale=.145]{images/ICSD2.png}}
\end{flushright}
\caption{
The illustration shows the intraclass distributions for each class. These distributions are created by applying softmax to the spatial dimension of the output prediction of the last layer of the network. As shown, the distribution of the sofa class is more similar to that of the chair than to the aeroplane, for example. These similarities between each pair of intraclass distributions have good potential for distillation. These distributions were created from the Pascal VOC 2012 dataset, which includes 21 category classes.}
\label{exp}
\end{figure}


For the purpose of training compact semantic segmentation networks, the knowledge distillation technique is investigated, which has already been tested and shown to be effective in classification tasks\cite{hinton2015distilling}\cite{romero2014fitnets}.
Like most existing methods, in this work, the semantic segmentation problem is approached by viewing it as a collection of distinct pixel classification problems. Then the knowledge distillation is applied to the pixel level. Different from the classification task, semantic segmentation has a structured output. Long-range dependencies are significant for semantic segmentation, and the teacher and student models typically capture different long-range contextual information due to the differences in the receptive fields.

In this work, we also present structured knowledge distillation and transfer the structure information with pair-wise distillation using intermediate feature maps, which are proven to contain rich information\cite{zhou2016learning}\cite{selvaraju2017grad}. This pair-wise distillation, along with the pixel-wise distillation, provides rich information for the student network from the teacher network.
To this end, an objective function that combines a conventional cross-entropy loss with the distillation losses is optimized.

In summary, the main contributions of this work are as follows:

\begin{itemize}
\item Proposing a new pairwise distillation method, Inter-Class Similarity Distillation (ICSD), to transfer structured informations from teacher to student.\\

\item Proposing a training strategy to control the the impact of distillation in training of the student network by adaptively changing the scale of losses (ALW).\\


\item Validating the effectiveness of the proposed method with extensive experiments on the Cityscapes and Pascal
VOC 2012 datasets with a state-of-the-art segmentation networks, DeepLab V3+ and PspNet.

\end{itemize}

==> temp/temp_related_work.tex <==
In the following, we review works of literature that are relevant to this work, including state-of-the-art researches on semantic segmentation and knowledge distillation.\\
\textbf{Semantic Segmentation:} Semantic segmentation is known as
a challenging task, which is about to combine global infor-
mation with detailed local information to predict the structure
of an input image in terms of classifying pixels to categories.
Semantic segmentation networks are generally larger than clas-
sification ones, as they have to extract additional information
beside the information needed for classification. The fully con-
volutional framework, first introduced in \cite{long2015fully}, added several
important improvements to segmentation network design. It
can use pretrained weights of classification networks, perform
on variable input size, and be trained end-to-end. 
DeepLabV3+\cite{chen2018encoder} and PSPNet\cite{zhao2017pyramid} are two of the most
powerful and popular existing segmentation networks. Due to
their flexible design, one can choose big and powerful or small
and efficient classifier networks as their backbones. They use
Atrous convolution and pyramid spatial pooling to capture
global context while preserving feature maps’ resolution and
details. In this work, DeepLab with ResNet101\cite{he2016deep} backbone
is adopted as the teacher and DeepLab with ResNet18 and MobileNet backbones
are chosen as the student networks.


In addition to cumbersome networks for highly accurate segmentation, real-time segmentation networks have been attracting increasingly more interest due to the need for real applications, such as mobile applications. This is because highly efficient segmentation networks can segment data in a fraction of the time as cumbersome networks. Most works concentrate on creating lightweight networks by speeding up the convolution operations using factorization methods. ENet\cite{yu2018bisenet}, inspired by\cite{chen2017rethinking}, incorporates multiple acceleration factors, such as multi-branch modules, early feature map resolution down-sampling, minimal decoder size, filter tensor factorization, etc. ESPNet\cite{mehta2018espnet} replaced conventional convolution layers with a spatial pyramid of dilated convolutions. ICNet\cite{zhao2018icnet} utilized cascading multi-resolution branches to increase efficiency. BiSeNet\cite{yu2018bisenet} uses two branches, one for learning spatial information and the other for obtaining a large receptive field: spatial and context paths. 


\textbf{Knowledge Distillation:} The idea of knowledge distillation
first appeared in\cite{hinton2015distilling}, where the student network uses the
teacher’s predictions as soft labels (compared to zero and one
hard label of ground-truth). Soft labels hold useful information
about the structure of a problem and relationships between
the categories and provide useful information for training the
student. The teacher and student framework is widely used for
helping to train compact students. There are also numerous
other scenarios where it comes useful. For instance, here is a list of some of the recent related works:
\begin{itemize}



\item {\cite{furlanello2018born} trains a sequence of identical networks in such a way that each network distills from the previously trained one and this leads to improved performance. }

\item{\cite{zhou2020channel} Makes use of a method of channel-wise distillation that enables students to mimic the correct outputs of the teacher.}

\item{\cite{chen2021distilling} Utilizes a review mechanism to use past feature maps as a guide for the current feature map's distillation. }

\item{\cite{sarridis2022indistill} Employs auxiliary models to hold pruned intermediate layers of teacher and student, then distills them using the curriculum learning approach.}

\item{\cite{liu2022transformer} proposes a relation-based knowledge distillation framework for transformers.}


\end{itemize}

Most of the discussed methods are designed for image classification, but \cite{li2017learning} applied its method for object detection as
well. Other examples of successful work on object detection and classification
include\cite{park2019relational}\cite{yue2020matching}\cite{tang2022distilling}\cite{yang2022prediction}\cite{chen2022knowledge}\cite{ye2022generalized}. After classification and detection, one of
the first applications of distillation to semantic segmentation
was introduced in\cite{ros2016training}. They used the prediction of the
teacher instead of the ground-truth for training the student.
It led to better results because the teacher’s output is an
easier distribution to learn. Due to the structural nature of semantic segmentation, additional distillation methods are applied in addition to pixel-wise knowledge distillation to transfer more structural information from teacher to student. Similar to\cite{zhou2020channel},\cite{liu2021exploring} attempts to take advantage of channel-wise distillation while employing a divide-and-conquer strategy because channel-wise distillation is time-consuming.\cite{wang2020intra} and \cite{feng2021double} try to transfer class-wise similarity by creating class prototypes and category-wise similarity by constructing the correlation matrix, respectively.\cite{xie2018improving} introduced the consistency loss between the student and the teacher to make their segmentation boundary similar. It also takes the L2 norm of the difference between the student's output probabilities and the teacher's as another loss. Authors of\cite{park2020knowledge} employed channel and spatial correlation loss function in addition to adaptive cross-entropy loss, which adaptively uses ground-truth labels and teacher predictions.\cite{heo2019comprehensive} investigated the design aspects of the feature distillation method by reviewing the position of feature maps to distill and distillation losses. They proposed a new distance function to distill meaningful information between the teacher and student using marginal ReLU.\cite{liu2019structured} introduced two novel
distillation losses in segmentation. Pairwise loss is defined as the mean square distance between elements of affinity matrices of the teacher and student networks (affinity matrix contains inner products between every pair of features which encode pixels). The second loss is called holistic distillation, which uses adversarial learning to make feature maps of student similar to its teacher’s, using a discriminator convolutional network.\cite{he2019knowledge} is another relevant work that was developed parallel
with\cite{liu2019structured}. It uses an affinity loss which is almost the same as
the pairwise loss in\cite{liu2019structured}, except that they train an auto-encoder
for the last convolutional layer of their teacher network before
computing its affinity matrix. They also use the direct L2 norm
distance between the student’s last convolutional features and
the teacher’s encoded features as an additional loss.

\begin{figure*}[htb]
\centerline{\includegraphics[scale=.40]{images/diagram.png}}
\caption{
Our proposed framework for knowledge distillation. The architecture of both the teacher and student networks is Deeplab-V3 +\cite{chen2018encoder}, although their encoders are different. Student network encoder depth is shallower than that of teacher network encoder depth. Teacher network is fixed the during the training process; only the student network will be trained with two distillation losses and cross-entropy loss. The pixel-wise distillation module uses the preReLU feature map of the last convolution layer of the decoder before probability scores to transfer detailed spatial information. The pair-wise distillation module uses the feature map of the last layer of the encoder to create a pair-wise similarity matrix and transfer global information.}
\label{fig}
\end{figure*}

In this paper, we use the idea of pre-activation pixel-wise distillation introduced in\cite{heo2019comprehensive} to distill the knowledge of the last convolution layer of the teacher to the student. Also, for transferring long-range information, a pair-wise distillation method is utilized, similar to\cite{liu2019structured} on the intermediate layers of teacher and student.
